Nimbus: Secure and Efficient Two-Party Inference for Transformers

Transformer models have gained significant attention due to their power in machine learning tasks. Their extensive deployment has raised concerns about the potential leakage of sensitive information during inference. However, when being applied to Transformers, existing approaches based on secure two-party computation (2PC) bring about efficiency limitations in two folds: (1) resource-intensive matrix multiplications in linear layers, and (2) complex non-linear activation functions like $\mathsf{GELU}$ and $\mathsf{Softmax}$. This work presents a new two-party inference framework $\mathsf{Nimbus}$ for Transformer models. For the linear layer, we propose a new 2PC paradigm along with an encoding approach to securely compute matrix multiplications based on an outer-product insight, which achieves $2.9\times \sim 12.5\times$ performance improvements compared to the state-of-the-art (SOTA) protocol. For the non-linear layer, through a new observation of utilizing the input distribution, we propose an approach of low-degree polynomial approximation for $\mathsf{GELU}$ and $\mathsf{Softmax}$, which improves the performance of the SOTA polynomial approximation by $2.9\times \sim 4.0\times$, where the average accuracy loss of our approach is 0.08\% compared to the non-2PC inference without privacy. Compared with the SOTA two-party inference, $\mathsf{Nimbus}$ improves the end-to-end performance of \bert{} inference by $2.7\times \sim 4.7\times$ across different network settings.

==> tex_files/Outline.tex <==
\section{Outline}


\subsection{Introduction}

The private inference of the deep neural network has emerging as a meaningful application, especially when the language models present powerful ability, such as ChatGPT~\cite{}....

Multi-party computation (MPC) techniques offer perfect privacy guarantee for both the client and server....

But the protection comes with substantial computation and communication costs for both linear and non-linear layers. \textcolor{red}{Linear}: The state-of-the-art of the HE linear protocol uses polynomial encoding of two matrices. However, they have low utilization ratio of the ciphertxt, leading to large communication cost of both the input and output ciphertexts. They also require expensive polynomial multiplication to simulate the computation of the inner product. \textcolor{red}{Non-linear}: The non-linear function suffers from high-order polynomial approximation or causes accuracy degradation of the model.


Therefore, to deal with the main bottleneck, our contributions on linear and non-linear functions are as follows.
\begin{itemize}
    \item Linear: \textcolor{red}{First, we notice a potential opportunity is to place the encryption weights at the client side for online computation.} \textcolor{red}{With this observation, the limitation of input communication is removed so that we can design more efficient protocol for the computation and compact output ciphertext.} 

    \item Non-linear: \textcolor{red}{We notice prior approximation of the non-linear function assign same importance to all input range.} Instead, we segment the pieces and fit each polynomial with distribution-ware optimization. We achieve much smaller order polynomial and pieces. Our method causes no accuracy degradation even without fine-tuning.
\end{itemize}
With these optimizations, we achieve around 6 to 10 times better run-time than Iron and Bumblebee.

\subsection{Preliminary}

\subsubsection{Transformer-based Models}

This section introduces the background of the transformer. 
\begin{itemize}
    \item Attention
    \item FFN
\end{itemize}

\subsubsection{Private Inference of Transformer Models}
\textbf{Notation, threat Model and security setup}

\textbf{HE-based Linear Protocol} 
\begin{itemize}
    \item Three stages overview: Input communication, HE-based Compute, Output communication.
    \item Polynomial encoding details.
    \item Low efficiency of three stages.
\end{itemize}



\textbf{Non-Linear Protocol} 
% backgroNon-nud
% 1. target bottleneck
% 2. target the bottleneck reason. Make the complexity relative, output computation sparisty->utilization ratio. 

% motivation
% 3. client-side computation->improve three stage utizi

% sec 
% 1. adv+problem
% 4.1 amortized overhead
% 4.2 client burden: computation commuication

% \subsection{Motivations}
% \textbf{Linear.} 
% \subsubsection{Inefficiency Analyasis of Linear Layer}
% \begin{itemize}
%     \item Evaluation metric: utilization ratio
%     \item Interdependence caused utilization problem
% \end{itemize}
% \subsubsection{Client-side Encrypted weight to Eliminate input communication}
% Based on the observation of relationship between token number, weight size and polynomial degree, we propose client-side encrypted weight scheme.
% \begin{itemize}
%     \item Remove cost of online input communication
%     \item Disentangle the interdependence
% \end{itemize}
% \subsubsection{Challenge of the client-side encrypted weight scheme}
% \begin{itemize}
%     \item Overall (amortized) overhead
%     \item Client side burden: memory and computation
% \end{itemize}


\subsection{Efficient Linear Layer Evaluation}
\subsubsection{Client-side Encrypted weight Scheme}
\begin{itemize}
    \item Low utilization problem of prior paradigm.
    \item Client-side encrypted weight paradigm as a solution.
\end{itemize}

\subsubsection{Efficient Scalar-vector HE Product}
1. Introduce the scalar-vector HE product.
\begin{itemize}
    \item Define row-wise encoding.
    \item Define scalar-vector multiplication.
    \item Rshift packing for Compact output ciphertext.
\end{itemize}
2. Complexity analysis.
\begin{itemize}
    \item Communication.
    \item Computation.
\end{itemize}

\subsubsection{Client burden Analysis}
The limited client may suffer from the heavy burden or prolong the latency.
\begin{itemize}
    \item Computation overhead: our method do not put much more burden to the client.
    \item memory: the extra overhead of memory can be overlapped by the communication.
\end{itemize}

% \subsubsection{SVD Optimization}
% We analyze the overhead for different weight shape and notice the $W_{h2}$ puts large burden to the client. Therefore, we use SVD to reduce the client burden and still bring acceleration.


\subsection{Distribution-aware Non-Linear Approximation}
To design the piece-wise polynomial of the non-linear function, we choose the critical points and fit each polynomial with the input distribution in mind.
\subsubsection{Exponential}
We design based on the exp input distribution.
\subsubsection{GELU}
We design based on the GELU input distribution.



\subsection{Evaluation}
\subsubsection{Experimental setup}
% \begin{itemize}
%     \item layer-type=linear, nonlinear
%     \item method=ours, bumblebee, iron, ciphergpt
%     \item network= (1Gbps, 0.1ms), (400Mbps, 5ms), (200Mbps, 10ms)
%     \item Client ability=32, 16, 8
%     \item poly-size=8192,4096
%     \item token=1, 32, 64, 128, 256, 512
%     \item Transformer model size= 768,1024,2048
% \end{itemize}

\subsubsection{Accuracy Results}

\subsubsection{End-to-end Performance and Breakdown}

\subsubsection{Client Burden Analysis}

\subsubsection{Amortized Overhead of Sending Encrypted Weights.}




\newpage

==> tex_files/backup.tex <==
The sparsity is a widely used property of the deep neural network~\cite{}.  It refers to the idea that small-magnitude weights do not contribute to the network's performance. Encouraging sparsity can lead to several benefits that make it a widely adopted practice. It reduces the size of the model and the computational costs. In the field of plaintext computation, pruning weights element-wisely has the maximum sparsity without compromising the model accuracy. However, one needs to increase the granularity to tailor the GPU computation for real acceleration, such as vector-wise sparsity and block-wise sparsity. Generally, the larger the granularity, the lower the sparsity to maintain the accuracy.

However, for the privately computed linear layer, the sparsity is hard to participate in. The linear layer is evaluated using homomorphic encryption, such as Gazelle~\cite{} or Cheetah~\cite{}. Gazelle evaluates the linear layer based on the SIMD encryption while the Cheetah encodes the values by polynomial. Their methods compute the matrix multiplication based on the dot product of two vectors. Therefore, the pruning needs to prune the row weight vector (or the diagonal weight) to bypass the computation. This is a really large granularity that slight pruning can lead to obvious accuracy degradation.

In this work, we improve the encoding scheme of both methods based on SIMD encoding and polynomial encoding. To better make use of the benefits of the small-granularity sparsity, we compute the matrix multiplication based on the outer product or partial sum for SIMD encoding and polynomial encoding, respectively. We next introduce them in order

\subsection{Improved SIMD Multiplication}
For the SIMD multiplication, besides the hardness of utilizing the sparsity, it also has the problem of rotation operation and the limited slot utility. In our method, besides addressing the cost of the rotation operation, we also improve the slot utility and utilize the sparsity. Our encoding scheme is illustrated in Figure \ref{fig:simd_matmul_illu}. 
\begin{figure}[tbp] 
  \centering
  \subfigure[The setting.]{\label{subfig:setting} \includegraphics[width=0.3\linewidth]{figures/methods/setting.png}}
  \subfigure[SIMD matmul based on the outer product.]{\label{subfig:simd_matmul}
  \includegraphics[width=0.65\linewidth]{figures/methods/simd_matmul.png}}
  \subfigure[The batched setting.]{\label{subfig:batched_setting}
  \includegraphics[width=0.3\linewidth]{figures/methods/batched_setting.png}}
  \subfigure[Batched SIMD matmul based on the outer product.]{\label{subfig:batched_simd_matmul}
  \includegraphics[width=0.65\linewidth]{figures/methods/batched_simd_matmul.png}}
  \caption{The illustration of the SIMD matrix multiplication based on the outer product.}
  \label{fig:simd_matmul_illu}
\end{figure}

\begin{figure}[tbp] 
  \centering
  \includegraphics[width=0.75\linewidth]{figures/methods/SIMD_illustration.png}
  \caption{The general illustration of how SIMD encodes the weight and activation matrices.}
  \label{fig:SIMD_illustration}
\end{figure}
The client encrypts values at the same position from different vectors into a ciphertext. The server expand a weight to the same length as the activation ciphertext. All the weights of the first column compute in the same way and the result construct the partial sum of the final result. Then we recurse for each hidden dimension to compute all partial sum and then sum them together as the final result. We detail the protocol in Algorithm \ref{alg:improved_SIMD_protocol}.
\begin{algorithm}[tb]
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    \caption{Secure Linear Protocol $\Pi_{\text {new\_SIMD}}$}
    \begin{algorithmic}[1]
        \REQUIRE Server and client hold share of the input $\ashare{\mathbf{X}}_{\mathrm{S}}, \ashare{\mathbf{X}}_{\mathrm{C}} \in \mathbb{Z}^{n \times k}_{p}$. Server also holds $\mathbf{W} \in \mathbb{Z}^{m \times n}_{p}$.
        Parameters for the window size $m_w=N/k, n_w=1, k_w=k$. Then the number of windows on every dimensions  $n^{\prime}=n, m^{\prime}=\left\lceil m / m_{\mathrm{w}}\right\rceil$, and $k^{\prime}=1$. Sparsity mask $mask \in \mathbb{Z}^{m^{\prime} \times n^{\prime}}_{2}$; 
        \ENSURE  Shares $\ashare{\mathbf{Z}}$, where $\mathbf{Z}=\mathbf{WX} \in \mathbb{Z}^{m \times k}_{p}$;
        \STATE Client partitions the matrix $\mathbf{X}$ into block matrices $\mathbf{X}_{\beta, \gamma} \in \mathbb{Z}_{p}^{n_{\mathrm{w}} \times k_{\mathrm{w}}}$ for $\beta \in\left[n^{\prime}\right]$ and $\gamma \in\left[k^{\prime}\right]$;

        \STATE Client repeats each row of $\mathbf{X}_{\beta, \gamma}$ for $m^{\prime}$ times as vectors $\mathbf{x}_{\beta, \gamma} \in \mathbb{Z}_{p}^{n_w \times m_w*k_w} (\mathbb{Z}_{p}^{n_w \times N})$;
        
        \STATE Client sends to server the ciphertexts $\left\{\mathrm{CT}_{\beta, \gamma}=\operatorname{Enc}\left(\hat{x}_{\beta, \gamma}\right)\right\}$;
        
        \STATE Server partitions the matrix $\mathbf{W}$ into vectors $\mathbf{W}_{\alpha, \beta} \in \mathbb{Z}_{p}^{m_w,n_w}$ and then expands each weight values of $\mathbf{W}_{\alpha, \beta}$ for $k_w$ times and obtains $\hat{w}_{\alpha, \beta} \in \mathbb{Z}_{p}^{n_w \times m_w*k_w} (\mathbb{Z}_{p}^{n_w \times N})$ for $\alpha \in\left[m^{\prime}\right]$ and $\beta \in\left[n^{\prime}\right]$. 
        Server samples $\mathbf{R} \in \mathbb{Z}_{p}^{m \times k}$ uniformly at random and partitions the matrix $\mathbf{R}$ into $\mathbf{r}_{\alpha, \gamma} \in \mathbb{Z}_{p}^{n_w \times m_w*k_w} (\mathbb{Z}_{p}^{n_w \times N})$;
        
        \STATE On receiving the ciphertexts $\left\{\mathrm{CT}_{\beta, \gamma}\right\}$ from client, server operates $\mathrm{CT}_{\alpha, \gamma}^{\prime}=\boxplus_{\beta \in\left[n^{\prime}\right]}\left(\hat{w}_{\alpha, \beta} \otimes \mathrm{CT}_{\beta, \gamma}\right) \boxminus \hat{r}_{\alpha, \gamma}$ for $\alpha \in\left[m^{\prime}\right]$ and $\gamma \in\left[k^{\prime}\right]$. Then server sends to client the ciphertexts $\left\{\mathrm{CT}_{\alpha, \gamma}^{\prime}\right\}$. Any computation of weight block with sparsity mask $mask_{\alpha, \beta}=0$ can be bypassed;
        \STATE Server outputs $\mathbf{R} \bmod p$ as the share $\langle\mathbf{Z}\rangle_0$;
        \STATE On receiving the ciphertexts $\left\{\mathrm{CT}_{\alpha, \gamma}^{\prime}\right\}$ from server, client computes $\left\langle\hat{z}_{\alpha, \gamma}\right\rangle_1=\operatorname{Dec}\left(\mathrm{CT}_{\alpha, \gamma}^{\prime}\right)$ that are decoded to $\langle\mathbf{Z}\rangle_1$;
        \RETURN $\ashare{\mathbf{Z}}$
        
    
    \end{algorithmic} 
\label{alg:improved_SIMD_protocol}
\end{algorithm}



Our benefits are listed as follows
\begin{itemize}
    \item Our method remove the rotation operation, which is the most expensive operation in SIMD-based matrix multiplication. 
    \item The utilized slots of the ciphertext equals the number of activaiton vectors. Compared to prior works that use the hidden dimension, our method can more freely improve the slot utility. The hidden dimension is fixed and the utility can become quite low if the model owns a small hidden dimension. For our method, the number of vectors are usually hundreds. Besides, the utility can be further imporved by batching inputs of the client. We also give the freedom of batching weight to further improve the utility, as illustrated in Figure \ref{subfig:batched_simd_matmul}. 
    \item Our method can deploy element-wise pruning. Any pruned weight can bypass one SIMD multiplication. Note that the batched weights increase the pruning granularit.
\end{itemize}


\subsection{Improved Cheetah Multiplication}
The original Cheetah (Iron)~\cite{} protocol for matrix multiplication encodes the weights and activations into windows. An example is shown in Figure \ref{fig:cheetah_matmul_illu}. Each polynomial multiplication uses a block of the weight matrix.
\begin{figure}[tbp] 
  \centering
  \subfigure[The setting.]{\label{subfig:cheetah_setting} \includegraphics[width=0.3\linewidth]{figures/methods/cheetah_setting.png}}
  \subfigure[Cheetah matmul based on the partial sum of the dot product.]{\label{subfig:cheetah_matmul}
  \includegraphics[width=0.65\linewidth]{figures/methods/cheetah_improved_matmul.png}}
  \caption{The illustration of the Cheetah matrix multiplication based on the partial sum of the dot product.}
  \label{fig:cheetah_matmul_illu}
\end{figure}

We define the protocol in Algorithm \ref{alg:improved_cheetah_protocol}.
\begin{algorithm}[tb]
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    \caption{Secure Linear Protocol $\Pi_{\text {new\_Cheetah}}$}
    \begin{algorithmic}[1]
        \REQUIRE Server and client hold share of the input $\ashare{\mathbf{X}}_{\mathrm{S}}, \ashare{\mathbf{X}}_{\mathrm{C}} \in \mathbb{Z}^{n \times k}_{2^{\ell}}$. Server also holds $\mathbf{W} \in \mathbb{Z}^{m \times n}_{2^{\ell}}$. Parameters for the window size $m_w=\sqrt{mN/kn}, n_w=\sqrt{nN/km}, k_w=k $. Then the number of windows on every dimensions  $n^{\prime}=\left\lceil n / n_{\mathrm{w}}\right\rceil, m^{\prime}=\left\lceil m / m_{\mathrm{w}}\right\rceil$, and $k^{\prime}=\left\lceil k / k_{\mathrm{w}}\right\rceil$. Sparsity mask $mask \in \mathbb{Z}^{m^{\prime} \times n^{\prime}}_{2}$; 
        \ENSURE  Shares $\ashare{\mathbf{Z}}$, where $\mathbf{Z}=\mathbf{WX} \in \mathbb{Z}^{m \times k}_{2^{\ell}}$;
        \STATE Client partitions the matrix $\mathbf{X}$ into block matrices $\mathbf{X}_{\beta, \gamma} \in \mathbb{Z}_{2^{\ell}}^{n_{\mathrm{w}} \times k_{\mathrm{w}}}$ for $\beta \in\left[n^{\prime}\right]$ and $\gamma \in\left[k^{\prime}\right]$;
        \STATE Client encodes the matrices to polynomials $\hat{x}_{\beta, \gamma}=\pi_R\left(\mathbf{X}_{\beta, \gamma}\right)$ for $\beta \in\left[n^{\prime}\right]$ and $\gamma \in\left[k^{\prime}\right]$. Then client sends to server the ciphertexts $\left\{\mathrm{CT}_{\beta, \gamma}=\operatorname{Enc}\left(\hat{x}_{\beta, \gamma}\right)\right\}$;
        \STATE Server partitions the matrix $\mathbf{W}$ into block matrices $\mathbf{W}_{\alpha, \beta} \in \mathbb{Z}_{2^{\ell}}^{m_{\mathrm{w}} \times n_{\mathrm{w}}}$. Server samples $\mathbf{R} \in \mathbb{Z}_{2^{\ell}}^{m \times k}$ uniformly at random and partitions the matrix $\mathbf{R}$ into $\mathbf{R}_{\alpha, \gamma} \in \mathbb{Z}_{2^{\ell}}^{m_{\mathrm{w}} \times k_{\mathrm{w}}}$;
        \STATE Server encodes the two block matrices to polynomials: 1) $\hat{w}_{\alpha, \beta} {=} \pi_L\left(\mathbf{W}_{\alpha, \beta}\right)$ for $\alpha \in\left[m^{\prime}\right]$ and $\beta \in\left[n^{\prime}\right]$, and 2) for $\alpha \in\left[m^{\prime}\right]$ and $\gamma \in\left[k^{\prime}\right]$, encoding $\mathbf{R}_{\alpha, \gamma}$ into $\hat{r}_{\alpha, \gamma}$;
        \STATE On receiving the ciphertexts $\left\{\mathrm{CT}_{\beta, \gamma}\right\}$ from client, server operates $\mathrm{CT}_{\alpha, \gamma}^{\prime}=\boxplus_{\beta \in\left[m^{\prime}\right]}\left(\hat{w}_{\alpha, \beta} \otimes \mathrm{CT}_{\beta, \gamma}\right) \boxminus \hat{r}_{\alpha, \gamma}$ for $\alpha \in\left[m^{\prime}\right]$ and $\gamma \in\left[k^{\prime}\right]$. Then server sends to client the ciphertexts $\left\{\mathrm{CT}_{\alpha, \gamma}^{\prime}\right\}$. Any computation of weight block with sparsity mask $mask_{\alpha, \beta}=0$ can be bypassed;
        \STATE Server outputs $\mathbf{R} \bmod 2^{\ell}$ as the share $\langle\mathbf{Z}\rangle_0$;
        \STATE On receiving the ciphertexts $\left\{\mathrm{CT}_{\alpha, \gamma}^{\prime}\right\}$ from server, client computes $\left\langle\hat{z}_{\alpha, \gamma}\right\rangle_1=\operatorname{Dec}\left(\mathrm{CT}_{\alpha, \gamma}^{\prime}\right)$ that are decoded to $\langle\mathbf{Z}\rangle_1$;
        \RETURN $\ashare{\mathbf{Z}}$
        
    
    \end{algorithmic} 
\label{alg:improved_cheetah_protocol}
\end{algorithm}

\begin{figure}[tbp] 
  \centering
  \includegraphics[width=0.75\linewidth]{figures/methods/cheetah_illustration.png}
  \caption{The general illustration of how Cheetah encodes the weight and activation matrices.}
  \label{fig:cheetah_illustration}
\end{figure}
A more general illustration of Cheetah-based protocol is in Figure \ref{fig:cheetah_illustration}. The window size of weights and activations are $(m_w,n_w)$ and $n_w,k_w)$, respectively. The constraint should be $m_wn_wk_w \leq N$, where N is the polynomial order. The number of communicated ciphertexts is $\frac{k}{k_w}\left(\frac{m}{m_w}+\frac{n}{n_w}\right)$. To minimize the communication ciphertexts, it is a constraint optimization problem. In the analysis of previous work, they usually set $n_k=n$ or search the optimal solution in brute-force fashion. This way is not friendly to the sparsity since only pruning the whole column of weights can bypass computation. Our goal is to shrink the granularity of the pruning as well as minimize the number of ciphertexts. We set $k_w=k$ so that it takes the most of the polynomial terms and we can use smallest window for weights. In this way, to minimize the $\frac{k}{k_w}\left(\frac{m}{m_w}+\frac{n}{n_w}\right)$ with $k_w=k$, we let $m_w=\sqrt{mN/kn}$ and $n_w=\sqrt{nN/km}$ to minimize the number of ciphertexts. In practice, the $m_w$ and $n_w$ are very small due to large $k_w$.

% In the original Cheetah, suppose each weight polynomial pack $\frac{N}{c_i}$ weights, then there are $\frac{c_i*c_o}{N}$ weight polynomials. Each activation polynomial pack one column of activation, then there are $n$ activation polynomials. Each weight polynomial needs to be multiplied with all activation polynomial, then there are $\frac{c_i*c_o*n}{N}$ polynomial multiplications. While in our method, we pack a $a*b$ weight block in a weight polynomial, where $b=\frac{N}{n}$ and $a=1$ (we can set it as 2 if a tricky way is allowed). There are $\frac{c_i*c_o}{a*b}=\frac{c_i*c_o*n}{a*N}$ weight polynomials. Each activation polynomial pack a $n*b$ block, and there are $\frac{c_i}{b}=\frac{c_i*n}{N}$ polynomials. Each weight polynomial only needs to be multiplied with one activation polynomial, then the number of polynomial multiplication is also $\frac{c_i*c_o*n}{N}$. Although our polynomial has smaller polynomial order, we achieve the same number of polynomial multiplication since we have higher coefficients utilization. If we integrate the sparsity, we can bypass the multiplication of the unused weights.



==> tex_files/rebuttal.tex <==
\begin{figure*}[htbp] 
  \centering
  % \subfigure[$4_{th}$ $\mathsf{Softmax}$ of BERT-base (MRPC).]{\label{subfig:bert_base_softmax_shallow} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-base-uncased_encoder.layer.0.attention.self.softmax_512.pdf}}
  % \subfigure[$4_{th}$ $\mathsf{GELU}$ of BERT-base (MRPC).]{\label{subfig:bert_base_gelu_shallow} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-base-uncased_encoder.layer.0.intermediate.intermediate_act_fn_512.pdf}}
  % \subfigure[$10_{th}$ $\mathsf{Softmax}$ of BERT-base (MRPC).]{\label{subfig:bert_base_softmax_deep} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-base-uncased_encoder.layer.11.attention.self.softmax_512.pdf}}
  % \subfigure[$10_{th}$ $\mathsf{GELU}$ of BERT-base (MRPC).]{\label{subfig:bert_base_gelu_deep} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-base-uncased_encoder.layer.11.intermediate.intermediate_act_fn_512.pdf}}
  
  \subfigure[$4_{th}$ $\mathsf{Softmax}$ of BERT-base (SQuAD).]{\label{subfig:bert_base_softmax_shallow} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-base-uncased_squad_encoder.layer.0.attention.self.softmax_512.pdf}}
  \subfigure[$4_{th}$ $\mathsf{GELU}$ of BERT-base (SQuAD).]{\label{subfig:bert_base_gelu_shallow} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-base-uncased_squad_encoder.layer.0.intermediate.intermediate_act_fn_512.pdf}}
  \subfigure[$10_{th}$ $\mathsf{Softmax}$ of BERT-base (SQuAD).]{\label{subfig:bert_base_softmax_deep} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-base-uncased_squad_encoder.layer.11.attention.self.softmax_512.pdf}}
  \subfigure[$10_{th}$ $\mathsf{GELU}$ of BERT-base (SQuAD).]{\label{subfig:bert_base_gelu_deep} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-base-uncased_squad_encoder.layer.11.intermediate.intermediate_act_fn_512.pdf}}
  
  \subfigure[$4_{th}$ $\mathsf{Softmax}$ of BERT-base (SWAG).]{\label{subfig:bert_base_softmax_shallow} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-base-uncased_swag_encoder.layer.0.attention.self.softmax_512.pdf}}
  \subfigure[$4_{th}$ $\mathsf{GELU}$ of BERT-base (SWAG).]{\label{subfig:bert_base_gelu_shallow} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-base-uncased_swag_encoder.layer.0.intermediate.intermediate_act_fn_512.pdf}}
  \subfigure[$10_{th}$ $\mathsf{Softmax}$ of BERT-base (SWAG).]{\label{subfig:bert_base_softmax_deep} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-base-uncased_swag_encoder.layer.11.attention.self.softmax_512.pdf}}
  \subfigure[$10_{th}$ $\mathsf{GELU}$ of BERT-base (SWAG).]{\label{subfig:bert_base_gelu_deep} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-base-uncased_swag_encoder.layer.11.intermediate.intermediate_act_fn_512.pdf}}
  
  % \subfigure[$4_{th}$ $\mathsf{Softmax}$ of BERT-large (MRPC).]{\label{subfig:bert_large_softmax_shallow} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-large-uncased_encoder.layer.0.attention.self.softmax_512.pdf}}
  % \subfigure[$4_{th}$ $\mathsf{GELU}$ of BERT-large (MRPC).]{\label{subfig:bert_large_gelu_shallow} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-large-uncased_encoder.layer.0.intermediate.intermediate_act_fn_512.pdf}}
  % \subfigure[$10_{th}$ $\mathsf{Softmax}$ of BERT-large (MRPC).]{\label{subfig:bert_large_softmax_deep} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-large-uncased_encoder.layer.10.attention.self.softmax_512.pdf}}
  % \subfigure[$10_{th}$ $\mathsf{GELU}$ of BERT-large (MRPC).]{\label{subfig:bert_large_gelu_deep} \includegraphics[width=0.23\linewidth]{figures/rebuttal/bert-large-uncased_encoder.layer.10.intermediate.intermediate_act_fn_512.pdf}}
  
  \subfigure[$4_{th}$ $\mathsf{Softmax}$ of GPT2 (wikitext-2).]{\label{subfig:gpt2_softmax_shallow} \includegraphics[width=0.23\linewidth]{figures/rebuttal/gpt2_h.0.attn.softmax_512.pdf}}
  \subfigure[$4_{th}$ $\mathsf{GELU}$ of GPT2 (wikitext-2).]{\label{subfig:gpt2_gelu_shallow} \includegraphics[width=0.23\linewidth]{figures/rebuttal/gpt2_h.4.mlp.act_512.pdf}}
  \subfigure[$10_{th}$ $\mathsf{Softmax}$ of GPT2 (wikitext-2).]{\label{subfig:gpt2_softmax_deep} \includegraphics[width=0.23\linewidth]{figures/rebuttal/gpt2_h.10.attn.softmax_512.pdf}}
  \subfigure[$10_{th}$ $\mathsf{GELU}$ of GPT2 (wikitext-2).]{\label{subfig:gpt2_gelu_deep} \includegraphics[width=0.23\linewidth]{figures/rebuttal/gpt2_h.10.mlp.act_512.pdf}}
  
  % \subfigure[$4_{th}$ $\mathsf{Softmax}$ of OPT-125m.]{\label{subfig:opt_125m_softmax_shallow} \includegraphics[width=0.23\linewidth]{figures/rebuttal/opt-125m_decoder.layers.0.self_attn.softmax_512.pdf}}
  % \subfigure[$4_{th}$ $\mathsf{GELU}$ of OPT-125m.]{\label{subfig:opt_125m_gelu_shallow} \includegraphics[width=0.23\linewidth]{figures/rebuttal/opt-125m_decoder.layers.4.activation_fn_512.pdf}}
  % \subfigure[$10_{th}$ $\mathsf{Softmax}$ of OPT-125m.]{\label{subfig:opt_125m_softmax_deep} \includegraphics[width=0.23\linewidth]{figures/rebuttal/opt-125m_decoder.layers.10.self_attn.softmax_512.pdf}}
  % \subfigure[$10_{th}$ $\mathsf{GELU}$ of OPT-125m.]{\label{subfig:opt_125m_gelu_deep} \includegraphics[width=0.23\linewidth]{figures/rebuttal/opt-125m_decoder.layers.10.activation_fn_512.pdf}}
  
  % \subfigure[$4_{th}$ $\mathsf{Softmax}$ of OPT-1.3b.]{\label{subfig:opt_1.3b_softmax_shallow} \includegraphics[width=0.23\linewidth]{figures/rebuttal/opt-1.3b_decoder.layers.8.self_attn.softmax_512.pdf}}
  % \subfigure[$4_{th}$ $\mathsf{GELU}$ of OPT-1.3b.]{\label{subfig:opt_1.3b_gelu_shallow} \includegraphics[width=0.23\linewidth]{figures/rebuttal/opt-1.3b_decoder.layers.8.activation_fn_512.pdf}}
  % \subfigure[$10_{th}$ $\mathsf{Softmax}$ of OPT-1.3b.]{\label{subfig:opt_1.3b_softmax_deep} \includegraphics[width=0.23\linewidth]{figures/rebuttal/opt-1.3b_decoder.layers.10.self_attn.softmax_512.pdf}}
  % \subfigure[$10_{th}$ $\mathsf{GELU}$ of OPT-1.3b.]{\label{subfig:opt_1.3b_gelu_deep} \includegraphics[width=0.23\linewidth]{figures/rebuttal/opt-1.3b_decoder.layers.10.activation_fn_512.pdf}}
  \caption{Supplementary materials for the question: generalization of insight on activation distribution to other models or datasets. We verify the activation distribution in other popular datasets. Specifically, we tested BERT-base on the SQuAD dataset (for question answering), and SWAG dataset (for multiple choice), and GPT2 on the Wikitext-2 dataset (for causal language modeling). Our findings show that the activation values exhibit obvious non-uniform distributions across different models and datasets. The distribution patterns are also similar for different models and datasets. For $\mathsf{Softmax}$, the most nonlinear part is close to zero and also has a higher density of values. For the $\mathsf{GELU}$, the majority of values are on the left side of zero. 
  % In comparison to the previous strategy of assuming a uniform input distribution, our approach of fitting nonlinear functions based on the activation distribution is expected to yield better results.
 }
\end{figure*}



\begin{figure*}[htbp] 
  \centering
  \subfigure[\#Token=16.]{\label{subfig:token16} \includegraphics[width=0.18\linewidth]{figures/rebuttal/bert-base-uncased_encoder.layer.0.intermediate.intermediate_act_fn_16.pdf}}
  % \subfigure[\#Token=32.]{\label{subfig:token32} \includegraphics[width=0.18\linewidth]{figures/rebuttal/bert-base-uncased_encoder.layer.0.intermediate.intermediate_act_fn_32.pdf}}
  \subfigure[\#Token=64.]{\label{subfig:token64} \includegraphics[width=0.18\linewidth]{figures/rebuttal/bert-base-uncased_encoder.layer.0.intermediate.intermediate_act_fn_64.pdf}}
  \subfigure[\#Token=128.]{\label{subfig:token128} \includegraphics[width=0.18\linewidth]{figures/rebuttal/bert-base-uncased_encoder.layer.0.intermediate.intermediate_act_fn_128.pdf}}
  \subfigure[\#Token=256.]{\label{subfig:token256} \includegraphics[width=0.18\linewidth]{figures/rebuttal/bert-base-uncased_encoder.layer.0.intermediate.intermediate_act_fn_256.pdf}}
  \subfigure[\#Token=512.]{\label{subfig:token512} \includegraphics[width=0.18\linewidth]{figures/rebuttal/bert-base-uncased_encoder.layer.0.intermediate.intermediate_act_fn_512.pdf}}
  \caption{Supplementary materials for the question: details about the batch size used to summarize the input distribution. The figures illustrate the input distribution of the $\mathsf{GELU}$ of BERT-base at the $4_{th}$ layer using MRPC dataset, with different numbers of tokens. We have observed that the distribution of intermediate activations becomes stable when the number of tokens exceeds 256. This observation holds true for other layers and models as well. Therefore, Nimbus selects a batch of data with a token count of 512 to summarize the input distribution of nonlinear functions.}
\end{figure*}



% Table generated by Excel2LaTeX from sheet 'results'
\begin{table*}[htbp]
  \centering
  \caption{Supplementary materials for the question: the performance comparison using $\mathsf{BOLT}$'s official codes. The experimental setup is the same as that of Figure 6, and the values are measured in seconds.}
    \begin{tabular}{ccccccccc}
    \toprule
    Method (LAN) & $L_{qkv}$ & $L_o$ & $L_{h1}$ & $L_{h2}$ & $GELU$ & $Softmax$ & $Others$ & $Total$ \\
    \midrule
    $\mathsf{BOLT}$ & 2.17  & 0.70  & 2.94  & 2.43  & 3.18  & 3.66  & 8.1   & 23.18 \\
    $\mathsf{Bumblebee}$ & 2.13  & 0.67  & 2.7   & 1.86  & 0.96  & 2.23  & 0.87  & 11.42 \\
    $\mathsf{Nimbus}$ & 0.17  & 0.06  & 0.25  & 0.26  & 0.28  & 0.56  & 0.87  & 2.45 \\
    \midrule
    Method (WAN) & $L_{qkv}$ & $L_o$ & $L_{h1}$ & $L_{h2}$ & $GELU$ & $Softmax$ & $Others$ & $Total$ \\
    \midrule
    $\mathsf{BOLT}$ & 2.38  & 0.81  & 3.30  & 2.67  & 22.20 & 23.16 & 28.12 & 82.64 \\
    $\mathsf{Bumblebee}$ & 2.54  & 0.76  & 3.42  & 1.98  & 3.36  & 9.01  & 1.95  & 23.02 \\
    $\mathsf{Nimbus}$ & 0.74  & 0.2   & 0.87  & 0.68  & 1.02  & 3.07  & 1.95  & 8.53 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%

